Autoencoders Learn Generative Linear Models

We provide a series of results for unsupervised learning with autoencoders. Specifically, we study shallow two-layer autoencoder architectures with shared weights. We focus on three generative models for data that are common in statistical machine learning: (i) the mixture-of-gaussians model, (ii) the sparse coding model, and (iii) the sparsity model with non-negative coefficients. For each of these models, we prove that under suitable choices of hyperparameters, architectures, and initialization, autoencoders learned by gradient descent can successfully recover the parameters of the corresponding model. To our knowledge, this is the first result that rigorously studies the dynamics of gradient descent for weight-sharing autoencoders. Our analysis can be viewed as theoretical evidence that shallow autoencoder modules indeed can be used as feature learning mechanisms for a variety of data models, and may shed insight on how to train larger stacked architectures with autoencoders as basic building blocks.

==> analysis.tex <==
\section{Learning untied weights}

Setup: The true, unknown dictionary is $A^* \in \R^{n \times m}$, and the random sample is generated as $y = A^*x^*$. Goal is learning to recover $A^*$ via sparse autoencoder with one hidden layer.

The hidden code $x = ReLU(W^{(1)}y + b)$ and $\hat{y} = W^{(2)}x$  where $W^{(1)} \in \R^{m \times n}, W^{(2)} \in \R^{n \times m}$ are weight matrices, and $b \in \R^m$ is the bias vector. Denote $z = W^{(1)}y + b$ the weighted sum before firing at hidden layer.

The squared error loss function: $L = \norm{y - \hat{y}}^2 = \norm{y -
  W^{(2)}x}^2$ for $x = ReLU(z)$.
%
We calculate the gradient of $L$ \wrt\ to the weights and biases. First, 
\begin{align*}
  \nabla_{W^{(2)}}L = -(y - W^{(2)}x)x^T
\end{align*}
%
This reminds us of the gradient of the same loss function in sparse coding given the current update. If we have nice properties of weights and biases, we may have nice descent property for $W^{(2)}$. The problem is that because of the bias $b$, $x$ cannot be assumed
zero-mean, the sign consistency of $x^*$ as in Arora ('15). We may only have the support consistency.
%
\begin{align*}
 \nabla_{b}L = -W^{(2)T}(y - W^{(2)}x)\circ Th(z)
\end{align*}
if $Th(z)$ is derivative of $RELU$ \wrt\ $z = W^{(1)}y + b$. Finally, the gradient \wrt\ $W^{(1)}$.
%
\begin{align*}
  \nabla_{W^{(1)}}L = -(W^{(2)T}(y - W^{(2)}x)\circ Th(z))y^T
\end{align*}
%
We'll consider the gradient update by column or row depending on which weight matrix is being updated. Given that $W^{(1)}$ is initialized with $A^{0T}$ and the second weights are
initial guess of the dictionary.

What to be shown?: Correlation property for $\nabla_{W_{i}^{(2)}}L$. The gradient of biases $\nabla_{b}L$ is bounded and $\nabla_{W_{i}^{(1)}}L$?


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> bias_update_nnsc.tex <==

The gradient of $L$ with respect to $b_i$ is
\begin{align*}
  \nabla_{b_i}L = -\sigma'(W_i^Ty + b_i)W_i^T(y - Wx)
\end{align*}
%
Similarly to the update for the weight matrix, we approximate this gradient with by replacing $\sigma'(W_i^Ty + b_i)$ with $\1_{x_i^* \neq 0}$, calculate the expected gradient and obtain:  $R = S \backslash \{i\}$
\begin{align*}
  (g_b)_i &= -\E[W_i^T(I - W_SW_S^T)y\1_{x_i^* \neq 0}]\\
          &= -\E[W_i^T(I - \sum_{j \in R}W_SW_S^T)\sum_{l \in S}A_l^*x_l^*\1_{x_i^* \neq 0}] \\
          &= -\E[W_i^T\sum_{l \in S}A_l^*x_l^*\1_{x_i^* \neq 0}]  + \E[\sum_{j \in R}W_SW_S^T)\sum_{l \in S}A_l^*x_l^*\1_{x_i^* \neq 0}] \\
          &=\E[W_i^T\sum_{j \in S}\cAj^*x_j^*\1_{x_i^* \neq 0}] - \E[W_i^T\sum_{j \in S}(W_j^Ty +
                      b_j)W_j\1_{x_i^* \neq 0}] \\
                   &= \E[\1_{i\in S}W_i^T\sum_{j,l \in S}x_l^*(W_j^T\cAl^*)W_j]  + \E[\1_{i\in S}W_i^T\sum_{j \in S}b_jW_j - \E[\1_{i\in S}W_i^T\sum_{j \in S}\cAj^*x_j^*] \\
                    &= \mux p_i\norm{W_i}^2\inprod{W_i}{\cAi^*} +
                      \mux \sum_{j \neq i}p_{ij}\norm{W_i}^2\inprod{W_i}{\cAj^*} + \mux \sum_{j \neq i}p_{ij}\inprod{W_i}{W_j}\inprod{W_j}{\cAi^*} \\
                    &+ \mux \sum_{j \neq i}p_{ij}\inprod{W_i}{W_j}\inprod{W_j}{\cAj^*} + \mux \sum_{j \neq l \neq i}p_{ijl}\inprod{W_i}{W_j}\inprod{W_j}{\cAl^*} \\
                    &+  p_i\norm{W_i}^2b_i + \sum_{j\neq i}p_{ij}\inprod{W_i}{W_j}b_j - \mux p_i\inprod{W_i}{\cAi^*} - \mux \sum_{j\neq i}p_{ij}\inprod{W_i}{\cAi^*} \\
                    &= p_ib_i + \sum_{j\neq i}p_{ij}\inprod{W_i}{W_j}b_j + \mux \sum_{j \neq i}p_{ij}\inprod{W_i}{W_j}\inprod{W_j}{\cAi^* + \cAj^*} + \mux \sum_{j \neq l \neq i}p_{ijl}\inprod{W_i}{W_j}\inprod{W_j}{\cAl^*}
\end{align*}

% Now, we attempt to study the gradient proxy by making use of the
% incoherence and closeness properties from which we expect that $\lambda_i =
% \inprod{W_i}{\cAi^*}$ is close to 1 and $\inprod{W_i}{\cAj^*}$ is small. We may also assume further about the distribution of $x^*$,
% e.g. constant expectation and variance $\mux , \sigmax  = O(1)$. Then,
% %
% \begin{align*}
%   \alpha_i = (\sigmax \lambda_i^2 + 2\mux b_i\lambda_i + b_i^2) p_i % + \sigmax 
%   % \norm{\diag(p_{ij})W_{-i}\cAi^*}^2 +
%   % 2\mux ^2\lambda_i\inprod{\cAi^*}{\sum_{j \neq i}p_{ij}W_j} +
%   + o(k^2/m^2)~\thanh{yet to work}
% \end{align*}
% %
% and
% \begin{align*}
%   \beta_i = \sigmax p_i\lambda_i % + (\sigmax \lambda_i + \mux b_i)(1-\norm{W_i}^2))
%   + o(k^2/m^2)~\thanh{yet to work}
% \end{align*}
% %
% Then, the proxy gradient has the following form:
% \begin{align*}
%   g_i = \sigmax p_i\lambda_i(W_i - \cAi^*) + \underbrace{(\sigmax \lambda_i^2 - \sigmax \lambda_i + 2\mux \lambda_ib_i + b_i^2)p_i}_{\tilde{\alpha}}W_i + \xi
% \end{align*}
% %
% where $\xi$ has norm bounded by (maybe) $o(k^2/m^2)$. The goal is to lower bound this gradient in terms of $\delta_i = \norm{W_i -
%   \cAi^*}$ and $\norm{g_i}$ itself. Denote $v = \tilde{\alpha}W_i + \xi$, then
% \begin{equation}
%   \label{eq:1}
%   g_i = 2\sigmax p_i\lambda(W_i - \cAi^*) + v
% \end{equation}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips18"
%%% End:


==> ica.tex <==

\section{ICA model with Laplace priors}
\subsection{Descent}
\label{sec:ica_dsc}

$\mux = 0$ and $var(x_i^*) = 2b^2 = \sigmax$. This case: set $\eta =
0$ noiseless case. The PDF of $x_i^*$:
\[
  \frac{1}{\sqrt{2\sigmax}}\exp\Bigl( -\sqrt{\frac{2}{\sigmax}}\abs{x}\Bigr)
\]

To simplify the analysis, we first study alternating minimization similar to sparse coding by alternating between estimating $x$ and updating $A$ with gradient descent. The analysis gives us understanding of the autoencoder for ICA.

We want to design a good approximate of the true gradient $\nabla_{A}{\mathcal{L}}_i = -\E[(y - Ax)x_i]$ as follows:

\begin{equation}
  \label{ica_eq:1}
  g_i = -\E[(y - Ax)\sgn(x_i)]
\end{equation}
%
% where $f$ is some function to be identified (\eg\ $\sgn(\cdot)$ in the
% sparse coding and expected to be $\1(\cdot)$ in this case). $f$ is
% such that $f(x_i) = f(x_i^*)$ with (very) high probability for the
% code $x = \thres_{C}(A^Ty)$. 
% Fact that 
% \[
%   1 = \1(\abs{x_i^*} \geq C + \alpha) + \1(\abs{x_i^*} \in [C-\alpha,
%   C + \alpha]) + \1(\abs{x_i^*} \leq C-\alpha)
% \]
Using Theorem~\ref{thm}: $\sgn(x_i) = \sgn(x_i^*)$ with high
probability for $x_i^* > C + \alpha = K$. Then,
%
\begin{align}
  g_i &= -\E[(y - Ax)\sgn(x_i)] \nonumber \\
      % &= \E[(y - Ax)\1(x_i \neq
      %   0)\1(\abs{x_i^*} \geq C + \alpha)] + \E[(y - Ax)\1(x_i \neq
      %   0)\1(\abs{x_i^*} \in [C-\alpha, C + \alpha])] \pm \gamma \\
      % &= -\E[(y - Ax)\sgn(x_i^*)\1(\abs{x_i^*} \geq C + \alpha)] - \E[(y - Ax)\sgn(x_i)\1(\abs{x_i^*} \in [C-\alpha, C + \alpha])] \pm \gamma
      &= -\E[(y - Ax)\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] - \E[(y - Ax)\sgn(x_i)\1(\abs{x_i^*} < K)] \pm \gamma
\end{align}
where $\gamma$ depends the failure probability quantified by Theorem~\ref{thm}.
Consider the first term and note that $x_j = A_j^Ty = A_j^TA^*x^*$ for $x_j
\neq 0$, so
\begin{align*}
  % g_i &= 
        \E[(y - Ax)\sgn(x_i^*)&\1(\abs{x_i^*} \geq K)] = \E[y\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] - \E[Ax\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] \\
      &= \E[A^*x^*\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] - \E[\sum_{j}A_jx_j\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] \\
      &= \E[A_i^*x_i^*\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] - \E[\sum_{j}A_jA_j^TA^*x^*\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)]
\end{align*}
since $x^*$ has independent, mean-zero entries. In fact, $\E[x_i^*\sgn(x_i^*)\1(\abs{x_i^*}
\geq K)]$, which depends on K (\ie\ $C$ and $\alpha$):
% = \E[x_i^*\1(\abs{x_i^*} \leq C + \alpha)]$ (somehow $p$ should be
% positive).
\begin{align*}
  \E[\abs{x_i^*}\1(\abs{x_i^*} \geq K)] &= (-x\exp(-\sqrt{2/\sigmax}x) - \sqrt{\sigmax/2}\exp(-\sqrt{2/\sigmax}x))\big\vert_{K}^{\infty} \\
                                                 &= (K + \sqrt{\sigmax/2})\exp(-\sqrt{2/\sigmax}K)
                                                   = (K + \sqrt{\sigmax/2})p
\end{align*}
for $p = \Prob[\abs{x_i^*} \geq K)] = \exp(-\sqrt{2/\sigmax}K)$
Then,
\begin{align*}
  g_i &= -(K+\sqrt{\sigmax/2})pA_i^* + \E[\sum_{j}A_jA_j^TA^*x^*\1[x_j \neq
        0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] - \E[(y - Ax)\sgn(x_i)\1(\abs{x_i^*} < K)] \pm \gamma
\end{align*}
%
We will further expand the second term: 
\begin{align*}
  \E[\sum_{j}A_jA_j^T&A^*x^*\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] \\
                     &= \E[A_iA_i^TA^*x^*\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] + \sum_{j \neq i}\E[A_jA_j^TA^*x^*\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] \pm \gamma \\
  &= (K+\sqrt{\sigmax/2})p\inprod{A_i}{A_i^*}A_i + \sum_{j \neq i}\E[A_jA_j^TA^*x^*\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq C + \alpha)] \pm \gamma 
\end{align*}
where in the last step we used $A^*x^* = \sum_{l}A_l^*x_l^*$ and independence of $x_l^*$'s and $x_i^*$. For any $j \neq i$, again we write % $\1(x_j \neq 0) = \1(\abs{x_j^*} \geq K) + \1(x_j \neq 0)\1(\abs{x_j^*} \in [C-\alpha, C + \alpha])$
with high probability:
\begin{align*}
  \E[A_jA_j^T&A^*x^*\1[x_j \neq 0]\sgn(x_i^*)\1(\abs{x_i^*} \geq K)] \\
             &= \E[A_jA_j^TA^*x^*\sgn(x_i^*)\1(\abs{x_j^*} \geq K, \abs{x_i^*} \geq K)] \\&+ 
               \E[A_jA_j^TA^*x^*\1(x_j \neq 0)\sgn(x_i^*)\1(\abs{x_j^*} < K
               )\1(\abs{x_i^*} \geq K)] \pm \gamma \\
             &= (K+\sqrt{\sigmax/2})pA_jA_j^TA_i^*\Prob[\abs{x_j^*} \geq K)] + \E[A_jA_j^TA^*x^*\1(x_j \neq 0)\sgn(x_i^*)\1(\abs{x_j^*} < K% \in [C-\alpha, C + \alpha]
               )\1(\abs{x_i^*} \geq K] \pm \gamma \\
             &= (K+\sqrt{\sigmax/2})p^2A_jA_j^TA_i^* + \E[A_jA_j^TA^*x^*\1(x_j \neq
               0)\sgn(x_i^*)\1(\abs{x_j^*} < K )\1(\abs{x_i^*} \geq K] \pm \gamma 
\end{align*}
% Here $\E[x_j^*\1[\abs{x_j^*} \geq C + \alpha) = 0$. Denote $q = \Prob[\abs{x_i^*} \geq C + \alpha)]$ depending on $(C, \alpha)$ and $\lambda_i = \inprod{A_i}{A_i^*}$
% (Remember that $\Prob[\abs{X} \geq t] = \exp(-\sqrt{2}t)$ for $X$ is a standard Laplace.)
Denote $\lambda_i = \inprod{A_i}{A_i^*}$ and put these together, we get
\begin{align*}
  g_i &=  (K+\sqrt{\sigmax/2})p(\lambda_iA_i - A_i^*) + (K+1)p^2\sum_{j \neq
        i}A_jA_j^TA_i^* - \E[(y - Ax)\sgn(x_i)\1(\abs{x_i^*} < K)] \\
        &+ \sum_{j \neq i}\E[A_jA_j^TA^*x^*\1(x_j \neq
               0)\sgn(x_i^*)\1(\abs{x_j^*} < K )\1(\abs{x_i^*} \geq K] \pm \gamma \\
      &= (K+\sqrt{\sigmax/2})p(\lambda_iA_i - A_i^*) + (K+1)p^2A_{-i}A_{-i}^TA_i^* - \E[(y - Ax)\sgn(x_i)\1(\abs{x_i^*} < K)] \\
        &+ \sum_{j \neq i}\E[A_jA_j^TA^*x^*\1(x_j \neq
               0)\sgn(x_i^*)\1(\abs{x_j^*} < K )\1(\abs{x_i^*} \geq K] \pm \gamma \\
\end{align*}
% We study first $p$ and $q$, then analyze the remaining perturbation terms.  and
% \begin{align*}
%   p = \E[x_i^*\1(\abs{x_i^*} \leq C + \alpha)] = 0
% \end{align*}
% that's why identify function doesn't work.

%
The perturbation terms left are:
\begin{align*}
  \E[(y - Ax)\1(x_i \neq 0)\1(\abs{x_i^*} < K)] % \in [C-\alpha, C + \alpha])]
\end{align*}
and,
\begin{align*}
  \E[A_jA_j^TA^*x^*\1(x_j \neq 0)\1(\abs{x_j^*} < % \in [C-\alpha, 
  K])\1(\abs{x_i^*} \geq K)]
\end{align*}
%
We will first bound $\Prob[x_i \neq 0 ~\&~ \abs{x_i^*} < K)]$ and
$\norm{y - Ax}$.
The remaining is to bound $\norm{y-Ax}$. Denote $S = \{j: \abs{x_j^*} \geq K\}$, then $k = |S|
\leq O(mp)$ \whp\ where $p= \Prob[\abs{x_j^*} \geq K]\}$ using
Chernoff bound (binomial random variable).

Denote $R = \{i \in
[m]\backslash S: x_i \neq
0\}$. $Ax = A_Sx_S + A_Rx_R = A_SA_S^Ty + A_RA_R^Ty = A_SA_S^TAx^*$ and 
\begin{align*}
  \norm{y - Ax} = \norm{(I - A_SA_S^T)A^*x^* } = \norm{(A_S^* - A_SA_S^TA_S^*)x_S^*} &\leq
                                                                 \norm{(I - A_SA_S^T)A^*}\norm{x^*} + \norm{A_RA_R^TA^*x^*} \\
  &\leq O(\delta mp)
\end{align*}
Moreover,
\begin{align*}
  \norm{A_S^* - A_SA_S^TA_S^*} &= \norm{(A_S^* - A_S + A_S(I- A_S^TA_S^*)} \\
                               &= \norm{(A_S^* - A_S + A_S(I- A_S^{*T}A_S^*) + (A_S - A_S^*)^TA_S^*)} \\
                               &\leq O(\delta\sqrt{k})
\end{align*}
since $A_S^{*T}A_S^* = I_k$
%

Therefore, we have
\[
  \norm{\E[(y - Ax)\1(x_i \neq 0)\1(\abs{x_i^*} < K)]} \leq O(2Kmp\exp(-(K - \lambda_iC)^2/8\sigma_{Z_i}^2))
\]

% How to pick $C$ (or $K$) such that $(K+1)p = (K+1)\exp(-\sqrt{2}K)
% \propto 1/n$

$p = \exp(-\sqrt{2/\sigmax}K) \propto 1/n$, or $K =
\Omega(\sqrt{\frac{\sigmax}{2}}\log n)$.

%  We study an upper bound of the probability:
% \begin{equation}
%   \label{eq:5}
%   \Prob[\abs{x_i^*  + Z_i} > C \big| \abs{x_i^*} \in [C-\alpha, C +
% \alpha])]
% \end{equation}
% and
% \begin{equation}
%   \label{eq:5}
%   \Prob[\abs{x_i^*} \in [C-\alpha, C + \alpha])] =
%   \exp(-\sqrt{2}(C-\alpha)) - \exp(-\sqrt{2}(C+\alpha)) = \exp(-\sqrt{2}C)(\exp(\sqrt{2}\alpha))- \exp(-\sqrt{2}\alpha))
% \end{equation}
%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips18"
%%% End:


==> init.tex <==
\section{Initialization}
\label{sec:init}

Our main result is a local analysis of the learning dynamics for two-layer autoencoders.
More specifically, we prove that the (batch) gradient descent linearly converges to the ground truth parameter $A$ given an initialization $W^0$ that is $O^*(1/\log n)$ column-wise close to the ground truth.
%In order to achieve such convergence, we assume a good initialization $W^0$ that is $O^*(1/\log n)$ colum-wise close to the ground truth.
Despite the fact that the recovery error at the convergence is exponentially better than the initial $1/\log n$ order, a natural question is how to achieve this initialization requirement.
%and if possible whether such initialization is even necessary.
In practice, random initialization for autoencoders is a common strategy and it often leads to surprisingly good results ~\cite{coates11_importance, saxe11_random}. In theory, however, the validity of the random initialization is still an open problem.
%We focus more on the first one regarding an initialization of the weights under the generative bilinear model.
For the $k$-sparse model, the authors in~\citep{arora15_neural} introduce an algorithm that provably produces such a coarse estimate of $A$ using spectral methods. This algorithm applies perfectly to this context of the autoencoder architecture.
%and certainly provides a guarantee that our results are non-trivial.
We conjecture that this spectral algorithm still works for non-negative sparse case (including the special mixture of Gaussian model) although, due to non-negativity, more complicated treatments including concentration arguments and sign flips of the columns are involved. We leave this to our future work.

% In the experiment, we will provide some 


==> plots.tex <==
\begin{figure}[!t]
\begin{center}
\resizebox{0.7\columnwidth}{!}{
%\begin{tabular}{ccc}
\begin{tikzpicture}[scale=1.2]
\begin{axis}[
		width=3.75cm,
		height=3cm,
		scale only axis,
		xmin=0, xmax=50,
		xlabel = {Iteration},
		xmajorgrids,
		ymin=0, ymax=1.2,
		ylabel={Reconstruction loss},
		ymajorgrids,
		line width=1.0pt,
		mark size=1.5pt,
		legend style={nodes={scale=0.75, transform shape},at={(0.50,.1)},anchor=south west,draw=black,fill=white,align=left}
		]
\addplot  [color=red,
		solid, 
		very thick,
		mark=o,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=1]{results/reconstruction_loss.txt};
\addlegendentry{$\sigma_{\eta} = 0.01$}
\addplot [color=blue,
		solid, 
		very thick,
		mark=square,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=2]{results/reconstruction_loss.txt};
\addlegendentry{$\sigma_{\eta} = 0.02$}
\addplot  [color=green,
		solid, 
		very thick,
		mark=star,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=3]{results/reconstruction_loss.txt};
\addlegendentry{$\sigma_{\eta} = 0.03$}
% \addplot [color=orange,
% 		solid, 
% 		very thick,
% 		mark=diamond*,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=4]{results/prob_success_sparfa_mc50_k6.txt};
% \addlegendentry{$\rho = 0.4$}
\end{axis}
\end{tikzpicture}
% &
% \begin{tikzpicture}[scale=1.2]
% \begin{axis}[
% 		width=3.75cm,
% 		height=3cm,
% 		scale only axis,
% 		xmin=0, xmax=50,
% 		xlabel = {Iteration},
% 		xmajorgrids,
% 		ymin= 0, ymax=.3,
% 		ylabel={Frobenious of the gradient},
% 		ymajorgrids,
% 		line width=1.0pt,
% 		mark size=1.0pt,
% 		legend style={nodes={scale=0.75, transform shape},at={(0.8,.65)},anchor=south,draw=black,fill=white,align=left}           
% 		]
% \addplot  [color=red,
% 		solid, 
% 		very thick,
% 		mark=o,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=1]{results/grad_norm.txt};
% \addlegendentry{$\sigma_{\eta} = 0.01$}
% \addplot [color=blue,
% 		solid, 
% 		very thick,
% 		mark=square,
% 		mark options={solid, scale=1.5},
% 		]
% 		table [x index = 0,y index=2]{results/grad_norm.txt};
% \addlegendentry{$\sigma_{\eta} = 0.02$}
% \addplot  [color=green,
% 		solid, 
% 		very thick,
% 		mark=star,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=3]{results/grad_norm.txt};
% \addlegendentry{$\sigma_{\eta} = 0.03$}
% % \addplot [color=orange,
% % 		solid, 
% % 		very thick,
% % 		mark=diamond*,
% % 		mark options={solid,scale=1.5},
% % 		]
% % 		table [x index = 0,y index=4]{results/error_sparfa_mc50_k6.txt};
% % \addlegendentry{$\rho = 0.4$}

% \end{axis}
% \end{tikzpicture}
% \end{tabular}
}
\caption{\small\sl The learning curve  in training step when the autoencoder is initialized by perturbing the ground truth. \label{fig_exp_perturb}}
\end{center}
\end{figure}
%}


==> plots_pca.tex <==
\begin{figure}[!t]
\begin{center}
\resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{ccc}
\begin{tikzpicture}[scale=1.2]
\begin{axis}[
		width=3.75cm,
		height=3cm,
		scale only axis,
		xmin=0, xmax=50,
		xlabel = {Iteration},
		xmajorgrids,
		ymin=0, ymax=1.2,
		ylabel={Reconstruction loss},
		ymajorgrids,
		line width=1.0pt,
		mark size=1.5pt,
		legend style={nodes={scale=0.75, transform shape},at={(0.50,.1)},anchor=south west,draw=black,fill=white,align=left}
		]
\addplot  [color=red,
		solid, 
		very thick,
		mark=o,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=1]{results/reconstruction_loss_pcab.5_4.txt};
\addlegendentry{$\sigma_{\eta} = 0.01$}
\addplot [color=blue,
		solid, 
		very thick,
		mark=square,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=2]{results/reconstruction_loss_pcab.5_4.txt};
\addlegendentry{$\sigma_{\eta} = 0.02$}
\addplot  [color=green,
		solid, 
		very thick,
		mark=star,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=3]{results/reconstruction_loss_pcab.5_4.txt};
\addlegendentry{$\sigma_{\eta} = 0.03$}
% \addplot [color=orange,
% 		solid, 
% 		very thick,
% 		mark=diamond*,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=4]{results/prob_success_sparfa_mc50_k6.txt};
% \addlegendentry{$\rho = 0.4$}
\end{axis}
\end{tikzpicture}
%&
%\begin{tikzpicture}[scale=1.2]
%\begin{axis}[
%		width=3.75cm,
%		height=3cm,
%		scale only axis,
%		xmin=0, xmax=50,
%		xlabel = {Iteration},
%		xmajorgrids,
%		ymin= 0, ymax=.3,
%		ylabel={Frobenious of the gradient},
%		ymajorgrids,
%		line width=1.0pt,
%		mark size=1.0pt,
%		legend style={nodes={scale=0.75, transform shape},at={(0.8,.65)},anchor=south,draw=black,fill=white,align=left}           
%		]
%\addplot  [color=red,
%		solid, 
%		very thick,
%		mark=o,
%		mark options={solid,scale=1.5},
%		]
%		table [x index = 0,y index=1]{results/grad_norm_pcab.5_4.txt};
%\addlegendentry{$\sigma_{\eta} = 0.01$}
%\addplot [color=blue,
%		solid, 
%		very thick,
%		mark=square,
%		mark options={solid, scale=1.5},
%		]
%		table [x index = 0,y index=2]{results/grad_norm_pcab.5_4.txt};
%\addlegendentry{$\sigma_{\eta} = 0.02$}
%\addplot  [color=green,
%		solid, 
%		very thick,
%		mark=star,
%		mark options={solid,scale=1.5},
%		]
%		table [x index = 0,y index=3]{results/grad_norm_pcab.5_4.txt};
%\addlegendentry{$\sigma_{\eta} = 0.03$}
% \addplot [color=orange,
% 		solid, 
% 		very thick,
% 		mark=diamond*,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=4]{results/error_sparfa_mc50_k6.txt};
% \addlegendentry{$\rho = 0.4$}
%\end{axis}
%\end{tikzpicture}
% \end{tabular}
}
\caption{\small\sl The learning curve  in training step when the autoencoder is initialized by PCA. \label{fig_exp_pca}}
\end{center}
\end{figure}
%}


==> plots_rand.tex <==
\begin{figure*}[!h]
\begin{center}
\resizebox{0.7\textwidth}{!}{
% \begin{tabular}{ccc}
\begin{tikzpicture}[scale=1.2]
\begin{axis}[
		width=3.75cm,
		height=3cm,
		scale only axis,
		xmin=0, xmax=50,
		xlabel = {Iteration},
		xmajorgrids,
		ymin=0, ymax=1.2,
		ylabel={Reconstruction loss},
		ymajorgrids,
		line width=1.0pt,
		mark size=1.5pt,
		legend style={nodes={scale=0.75, transform shape},at={(0.50,.1)},anchor=south west,draw=black,fill=white,align=left}
		]
\addplot  [color=red,
		solid, 
		very thick,
		mark=o,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=1]{results/reconstruction_loss_randb.5_1.txt};
\addlegendentry{$\sigma_{\eta} = 0.01$}
\addplot [color=blue,
		solid, 
		very thick,
		mark=square,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=2]{results/reconstruction_loss_randb.5_1.txt};
\addlegendentry{$\sigma_{\eta} = 0.02$}
\addplot  [color=green,
		solid, 
		very thick,
		mark=star,
		mark options={solid,scale=1.5},
		]
		table [x index = 0,y index=3]{results/reconstruction_loss_randb.5_1.txt};
\addlegendentry{$\sigma_{\eta} = 0.03$}
% \addplot [color=orange,
% 		solid, 
% 		very thick,
% 		mark=diamond*,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=4]{results/prob_success_sparfa_mc50_k6.txt};
% \addlegendentry{$\rho = 0.4$}
\end{axis}
\end{tikzpicture}
% &
% \begin{tikzpicture}[scale=1.2]
% \begin{axis}[
% 		width=3.75cm,
% 		height=3cm,
% 		scale only axis,
% 		xmin=0, xmax=50,
% 		xlabel = {Iteration},
% 		xmajorgrids,
% 		ymin= 0, ymax=.3,
% 		ylabel={Frobenious of the gradient},
% 		ymajorgrids,
% 		line width=1.0pt,
% 		mark size=1.0pt,
% 		legend style={nodes={scale=0.75, transform shape},at={(0.8,.65)},anchor=south,draw=black,fill=white,align=left}           
% 		]
% \addplot  [color=red,
% 		solid, 
% 		very thick,
% 		mark=o,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=1]{results/grad_norm_randb.5_1.txt};
% \addlegendentry{$\sigma_{\eta} = 0.01$}
% \addplot [color=blue,
% 		solid, 
% 		very thick,
% 		mark=square,
% 		mark options={solid, scale=1.5},
% 		]
% 		table [x index = 0,y index=2]{results/grad_norm_randb.5_1.txt};
% \addlegendentry{$\sigma_{\eta} = 0.02$}
% \addplot  [color=green,
% 		solid, 
% 		very thick,
% 		mark=star,
% 		mark options={solid,scale=1.5},
% 		]
% 		table [x index = 0,y index=3]{results/grad_norm_randb.5_1.txt};
% \addlegendentry{$\sigma_{\eta} = 0.03$}
% % \addplot [color=orange,
% % 		solid, 
% % 		very thick,
% % 		mark=diamond*,
% % 		mark options={solid,scale=1.5},
% % 		]
% % 		table [x index = 0,y index=4]{results/error_sparfa_mc50_k6.txt};
% % \addlegendentry{$\rho = 0.4$}

% \end{axis}
% \end{tikzpicture}
% \end{tabular}
}
\caption{\small\sl The learning curve  in training step when the autoencoder is randomly initialized. \label{fig_exp_rand}}
\end{center}
\end{figure*}
%}

